On-Demand Delivery from Stores: Dynamic Dispatching and Routing with Random Demand

On-demand delivery has become increasingly popular around the world. Motivated by a large grocery chain store who offers fast on-demand delivery services, we model and solve a stochastic dynamic driver dispatching and routing problem for last-mile delivery systems where on-time performance is the main target. The system operator needs to dispatch a set of drivers and specify their delivery routes facing random demand that arrives over a fixed number of periods. The resulting stochastic dynamic program is challenging to solve due to the curse of dimensionality. We propose a novel structured approximation framework to approximate the value function via a parametrized dispatching and routing policy. We analyze the structural properties of the approximation framework and establish its performance guarantee under large-demand scenarios. We then develop efficient exact algorithms for the approximation problem based on Benders decomposition and column generation, which deliver verifiably optimal solutions within minutes. The evaluation results on a real-world data set show that our framework outperforms the current policy of the company by 36.53% on average in terms of delivery time. We also perform several policy experiments to understand the value of dynamic dispatching and routing with varying fleet sizes and dispatch frequencies.

==> latexmacro.tex <==
\RequirePackage{amsmath,amssymb,bm}

%************************-begin-operators
%

\DeclareMathOperator{\pr}{\mathbb P}
\DeclareMathOperator{\E}{\mathbb E}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Corr}{Corr}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\ind}{\mathbb I}
%\DeclareMathOperator*{\argmin}{argmin}
%\DeclareMathOperator*{\argmax}{argmax}
\def\ud{\mathrm{d}}
\def\Real{\mathbb R}
\def\Int{\mathbb Z}
\def\NatInt{\mathbb N}

%
%************************-end-operators
%
%
%************************-begin-bold math letters
%
\def\BFA{\bm A}
\def\BFa{\bm a}
\def\BFB{\bm B}
\def\BFb{\bm b}
\def\BFC{\bm C}
\def\BFc{\bm c}
\def\BFD{\bm D}
\def\BFd{\bm d}
\def\BFE{\bm E}
\def\BFe{\bm e}
\def\BFF{\bm F}
\def\BFf{\bm f}
\def\BFG{\bm G}
\def\BFg{\bm g}
\def\BFH{\bm H}
\def\BFh{\bm h}
\def\BFi{\bm i}
\def\BFI{\bm I}
\def\BFJ{\bm J}
\def\BFj{\bm j}
\def\BFK{\bm K}
\def\BFk{\bm k}
\def\BFL{\bm L}
\def\BFl{\bm l}
\def\BFM{\bm M}
\def\BFm{\bm m}
\def\BFN{\bm N}
\def\BFn{\bm n}
\def\BFO{\bm O}
\def\BFo{\bm o}
\def\BFP{\bm P}
\def\BFp{\bm p}
\def\BFQ{\bm Q}
\def\BFq{\bm q}
\def\BFR{\bm R}
\def\BFr{\bm r}
\def\BFS{\bm S}
\def\BFs{\bm s}
\def\BFT{\bm T}
\def\BFt{\bm t}
\def\BFU{\bm U}
\def\BFu{\bm u}
\def\BFV{\bm V}
\def\BFv{\bm v}
\def\BFW{\bm W}
\def\BFw{\bm w}
\def\BFX{\bm X}
\def\BFx{\bm x}
\def\BFY{\bm Y}
\def\BFy{\bm y}
\def\BFZ{\bm Z}
\def\BFz{\bm z}
%
% bold face arabic numbers 
%
\def\BFzero{\bm 0}
\def\BFone{\bm 1}
\def\BFtwo{\bm 2}
\def\BFthree{\bm 3}
\def\BFfour{\bm 4}
\def\BFfive{\bm 5}
\def\BFsix{\bm 6}
\def\BFseven{\bm 7}
\def\BFeight{\bm 8}
\def\BFnine{\bm 9}
%
% bold face Greek letters
%
\def\BFalpha{\pmb \alpha}
\def\BFbeta{\pmb \beta}
\def\BFgamma{\pmb\gamma}
\def\BFGamma{\pmb \Gamma}
\def\BFdelta{\pmb \delta}
\def\BFDelta{\pmb \Delta}
\def\BFepsilon{\pmb\epsilon}
\def\BFvarepsilon{\pmb\varepsilon}
\def\BFzeta{\pmb \zeta}
\def\BFeta{\pmb\eta}
\def\BFtheta{\pmb \theta}
\def\BFTheta{\pmb \Theta}
\def\BFvartheta{\pmb \vartheta}
\def\BFiota{\pmb \iota}
\def\BFkappa{\pmb \kappa}
\def\BFlambda{\pmb\lambda}
\def\BFLambda{\pmb \Lambda}
\def\BFmu{\pmb \mu}
\def\BFnu{\pmb \nu}
\def\BFxi{\pmb \xi}
\def\BFXi{\pmb \Xi}
\def\BFpi{\pmb \pi}
\def\BFPi{\pmb \Pi}
\def\BFrho{\pmb \rho}
\def\BFvarrho{\pmb \varrho}
\def\BFsigma{\pmb \sigma}
\def\BFSigma{\pmb \Sigma}
\def\BFtau{\pmb \tau}
\def\BFupsilon{\pmb\upsilon}
\def\BFUpsilon{\pmb\Upsilon}
\def\BFphi{\pmb \phi}
\def\BFvarphi{\pmb \varphi}
\def\BFPhi{\pmb \Phi}
\def\BFchi{\pmb \chi}
\def\BFpsi{\pmb \psi}
\def\BFPsi{\pmb \Psi}
\def\BFomega{\pmb \omega}
\def\BFOmega{\pmb \Omega}
%
%************************-end-bold math letters
%

